Scheduling for Weighted Flow and Completion Times in Reconfigurable Networks

New optical technologies offer the ability to reconfigure network topologies dynamically, rather than setting them once and for all. This is true in both optical wide area networks (optical WANs) and in datacenters, despite the many differences between these two settings. Because of these new technologies, there has been a surge of both practical and theoretical research on algorithms to take advantage of them. In particular, Jia et al. [INFOCOM '17] designed online scheduling algorithms for dynamically reconfigurable topologies for both the makespan and sum of completion times objectives. In this paper, we work in the same setting but study an objective that is more meaningful in an online setting: the sum of flow times. The flow time of a job is the total amount of time that it spends in the system, which may be considerably smaller than its completion time if it is released late. We provide competitive algorithms for the online setting with speed augmentation, and also give a lower bound proving that speed augmentation is in fact necessary. As a side effect of our techniques, we also improve and generalize the results of Jia et al. on completion times by giving an $O(1)$-competitive algorithm for arbitrary sizes and release times even when nodes have different degree bounds, and moreover allow for the weighted sum of completion times (or flow times).

==> conc.tex <==
c

==> stashed-proof.tex <==
Recall that $\mathcal S(t)$ includes all released and unsatisfied jobs at time $t$. At any point in time $t$, we write an upper bound on the remaining cost that the algorithm will incur for jobs in $\mathcal S(t)$.  This upper bound accounts for the remaining weighted flow time of the jobs in the system assuming no more jobs arrive.  That is defined as follows,
$$R(t) := \sum_{i \in \mathcal S(t)} w_i \left (\sum_{j \in U_i, w_i < w_j} \frac{1}{sd_{u_i}} + \sum_{j \in V_i, w_i < w_j} \frac{1}{sd_{v_i}}   \right )$$

This is the maximum remaining cost due to the following.  Fix a job $i \in \mathcal S(t)$.  This job will contribute its  weight $w_i$ to the objective on each remaining time step the job is alive.  The two inner terms state that  job $i$ waits on the higher weight jobs adjacent to $u_i$ and $v_i$.    These jobs are processed at a rate of $sd_{u_i}$ and $sd_{v_i}$, respectfully. In the worst case,  nodes $u_i$ and $v_i$ are busy at separate time steps.  Note that if neither are busy then we  process $i$ and the job is completed.  Thus this upper bounds the waiting time.

To show the lemma, we will bound the total increase in this approximate remaining cost as jobs arrive.  We claim that   $2\alpha_i$ is  exactly the increase in $R(t)$   due to $i$'s arrival.  Consider the first two terms of $2\alpha_i$.  That is, 
\begin{eqnarray*}
&&\frac{1}{sd_{u_i}} \left (  w_i \sum_{j \in U_i(t), w_i <  w_j}   1 +   \sum_{j \in U_i(t), w_i > w_j} w_j \right )  \\
\end{eqnarray*}

This corresponds to the interactions happening at node $u_i$ due to $i$'s arrival.  The first term states that job $i$ need only wait on jobs that have higher weight than $i$ and these jobs are processed at a rate of $s d_{u_i}$.  The second term accounts for all lower weight jobs waiting on $i$.  The second two terms of $2\alpha_i$ are analogous for node $v_i$.   

Knowing that $ \alpha_i$ exactly accounts for the increase in  $R(t)$ when $i$ arrives, $\sum_i 2\alpha_i$ is an upper bound on the algorithm's objective and the lemma follows.  
%More formally, let $A(t)$ denote the remaining cost of the algorithm (with speed $s$) on the jobs in $\mathcal S(t)$.  So by the above discussion, we know that $A(t) \leq R(t)$ for all $t$.  For all jobs $i$, let $A(i)$ denote  the increase in the true cost of the algorithm due to job $i$'s arrival, i.e., $A(i) = A(r_i) - A(r_i-1)$ \mdnote{if arrival times are unique?}  Then we have that  
%\begin{align*}
%    ALG(s) &= \sum_{i} (A(r_i) - (A(r_{i}) - 1))
%\end{align*}

\mdnote{This seems vague.  In particular, it doesn't actually refer to $R(t)$ anywhere.  I'd like to be more explicit if possible to really get the desired equation.} \bmnote{ah.  It should be $R(t)$, does it sound better now?} \mdnote{I think what's not explicit is how $R(t)$ relates to $ALG(s)$.  As you say, it's definitely an upper bound if nothing else arrives.  But other things are arriving.  So I think you've definitely shown that a) $2\alpha_i$ is the increase in $R(t)$ when $i$ arrives, and b) $R(t)$ is an upper bound on the remaining cost of $ALG$ if nothing else shows up.  But how do  you go from those facts to get that $\sum_{i \in \mathcal S} \alpha_i \geq \frac12 ALG(s)$? I think there's something obvious I'm missing.}
\end{proof}
